A modern approach to String Amplitudes and Intersection Theory

In this thesis, we study the properties of String theory amplitudes within the framework of Intersection Theory (IT) for twisted (co)homology, which, as recently proposed, offered a novel approach to analyze relations between scattering amplitudes, in string theory as well as in QFT. As only recently pointed out, thanks to IT, the analytic properties of scattering amplitudes can be related to the topological properties of the manifolds characterizing their integral representation. Tree-level string amplitudes, as well as Feynman integrals, obey both linear and quadratic relations governed by intersection numbers, which act as scalar products between vector spaces. We show how (co)homology with values in a local system allows to interpret closed strings tree amplitudes as intersection numbers between twisted cocycles, and open strings tree amplitudes as parings between a twisted cocycle and a twisted cycle. We present different algorithms to evaluate univariate and multivariate intersection numbers between both log and non-log twisted cocycles. We explore a diagrammatic method for the computation of intersection number between twisted cycles of the moduli space of the n-punctured Riemann sphere. We use IT to rederive Kawai-Lewellen-Tye (KLT) relations, naturally emerging as a twisted version of Riemann period relations. We compute intersection matrix between 2D twisted cycles to explicitly obtain the KLT decomposition of five closed tachyons tree amplitudes into partial five open tachyons tree amplitudes. We explicitly determine the intersection matrix between 2D Parke-Taylor (PT) forms. We use a recursive algorithm for generic n cocycle intersection numbers to project tachyon amplitudes integrand into a PT basis, and we apply it to the scattering of four and five tachyons. The methods discussed in the thesis can be broadly applied to problems involving Aomoto-Gelfand integrals.

==> extra.tex <==
Scattering amplitudes, describing transition probabilities among asymptotic quantum states, are the key objects of perturbative approach to quantum field theory (QFT), and they therefore appear in all branch of physics, from Cosmology to Condensed Matter Physics, from Nuclear to Particle Physics. Thanks to Feynman diagrammatic interpretation of Dyson series, one is quite easily able to write down loop by loop contributions, however their evaluation is in general a vary challenging task, due both to convergency problems and to the increasing number of diagrams one has to consider at higher orders.
Many techniques have been developed to perform such integrals, and it has been discovered they actually turn not to be independent; many relations among them have been found and explored along the last decades, as color-kinematic double copies (\cite{2008},\cite{BCJ}) and integration by part identities (IBPs), based, under some assumptions, on the null contribution of surface terms, (\cite{TKACHOV198165},\cite{Chetyrkin1981IntegrationBP}). These relations induce a vector structure on amplitude space, allowing one to identify a minimal set of integrals, known as Master Integrals, in terms of which one can decompose all other integral, as in ordinary algebra. Finding a proper basis of such space and evaluating coefficients for the decomposition onto them allows one both to drastically reduce computational effort and to investigate more deeply features of the theory structure. 
The classical way to perform Master integral decomposition through integration by parts identities is the Laporta Algorithm \cite{2000}.
Recently it has been found (\cite{Mizera:2017rqa}, \cite{Frellesvig:2019kgj},\cite{Frellesvig:2019uqt},\cite{Frellesvig:2020qot},\cite{Mastrolia:2018uzb}) that such a decomposition can be achieved by means of a geometric algebraic theory called Intersection Theory (\cite{1997HypergeometricFM},\cite{Aomoto},\cite{Mimachi},\cite{Mimachi:2002gi}\cite{Mimachi:2004ez}).
According to Aomoto-Gelfand interpretation, an integral can be seen as a pairing between a form, the integrand, and a path, the contour of integration; by Stokes' theorem we know that there are several forms that, paired with a given contour, give the same integral, as well as many contours that, paired with a given form, leave the integral unchanged; this means that integrals are indeed pairings among equivalence classes: equivalence classes of forms are known as cocycles and equivalence classes of paths are called cycles.
The spaces of cocycles and cycles of a given dimension are endowed by a group structure and they are respectively named homology group and cohomology group.

By defining suitable dual spaces of co-homology spaces, one is able to introduce two non degenerate bilinear pairings called intersection numbers. This suggestive name is due to the fact that in considering ordinary homology, the scalar product among cycles is actually just their geometrical intersection.
graph polynomial
The key objects of intersection theory are therefore intersection numbers among cycles, intersection numbers among cocycles and parings between cycles and cocycles. These quantities turn not to be independent, but related by both linear (Contiguity relations) and quadratic relations (Riemann period relations).

Feynman integrals as well as String amplitudes, via Koba-Nielsen factor, involve multivalued functions, polynomials to some non integer power; in order for intersection theory to be applied one has to suitable choose homology and cohomology;  different choices are possible, as relative co-homology or intersection co-homology, but actually it is not still clear which one should provide the most appropriate description; in this thesis we explore the possibility to use the so called twisted co-homology, defined on a proper line bundle on the integration domain, called Local system  (\cite{10.2307/1969099},\cite{10.1007/978-3-0346-0209-9_5}).

The evaluation of intersection numbers for univariate twisted forms require the solution of differential equations and the application of Cauchy’s residue theorem. The multivariate case is instead more involving: twisted cocycles intersection is  if twisted cocycles only have simple poles and they can be written as differential of logarithmic forms, their intersection number can be evaluated by a generalized version of Residue theorem as elaborated by Matsumoto (\cite{Matsumoto1998IntersectionNF}) or Mizera (\cite{Mizera:2017rqa}); for general forms the evaluation of the intersection number turns to be a more challenging task, in \cite{Frellesvig:2019uqt} a recursive method is proposed, 


In this thesis we apply intersection language to tree level bosonic string amplitudes (\cite{zwiebach_2004},\cite{Polchinski:1998rq},\cite{kiritsis:in2p3-00714916},\cite{Green:2012oqa},\cite{Green:2012pqa},\cite{Tong:2009np},\cite{Staessens:2010vi}). Since Maxwell unified electric and magnetic phenomena under a same framework, physicist have been inspired to try describing all nature forces by the same language: electroweak theory, developed by Glashow, Salam and Weinberg, achieved unify electromagnetism and weak interaction, while quantum cromodynamics, although not properly unify strong interaction, at least provides a description in terms of a quantum field theory coherently to electroweak interpretation. On the other hand, gravity is described by a classical and completely different theory: General Relativity. The attempt to also describe gravitational interaction into a quantum framework is one of the most fascinating task of theoretical physics.
String theory is, at the moment, one of the best candidates to describe nature at scales where we suppose gravity should enter into processes comparably to other forces; the basic idea behind string theory is to consider fundamental objects of the nature not as pointlike particles but as extended one-dimensional strings. 
The simplest string theory one can consider is the bosonic string theory, containing only bosonic degrees of freedom,  in order for classical symmetries to be preserved at quantum level 


The multivariate case is instead more involving. If twisted cocycles only have simple poles and they can be written as differential of logarithmic forms, their intersection number can be evaluated by a generalized version of Residue theorem as elaborated by Matsumoto \cite{Matsumoto1998IntersectionNF} or Mizera \cite{Mizera:2017rqa}. For general multivariate forms the computation of the intersection number turns to be a still more challenging task; Frellesvig, Gasparotto, Mandal, Mastrolia, Matiazzi and Mizera  \cite{Frellesvig:2019uqt} proposed a recursive method based into the reiterative reduction of the dimensionality of the intersection number by solving suitable differential equations. \\

The classical way to add matter is imposing supersymmetry, this procedure remarkably eliminates tachyonic states and reduces critical dimension to $D=10$.
Bosonic string theory turns to be a useful toy model: tree level amplitudes in bosonic and supersymmetric string theory shares the same structure, due to the decoupling of fermionic degrees of freedom only contributing to an overall factor. Notice that when one considers high genera wordlsheets this is in general no long true,  
Closed $n$ strings amplitudes at order $g$ are defined as integrals over the Moduli space of the $n-$ punctured Riemann surface of genus $g$, while open $n$ strings amplitudes at order $g$ as integrals over the Moduli space of the 
Focusing on tree level amplitudes, the intristing spaces are then the Moludi space of the punctured sphere and the one of the disk with $n$ punctured along the boundary. 

The interest in considering string amplitudes is not a mere ontological lucubration or a mathematical divertissement, it turns to be a vary useful tool to investigate quantum field amplitudes structure: many duality relations among QFT amplitudes, often conjectured, can be elegantly obtained as pointlike limit of strings dualities, for instance double copy duality expressing quantum gravity amplitudes as two Yang-Mills amplitudes can be seen as a KLT decomposition of closed massless string amplitudes (graviton) into two partial open massless strings amplitudes (gluons). This fact suggests the possibility to find new relations among QFT amplitudes by better undestanding string amplitudes structure and by exploring new duality relations among them.


In the last couple of years, there has been an intense development of novel mathematical ideas related to the application of intersection theory to amplitudes in QFT. 

 The only simple case is for logarithmic (dlog) differential forms, which bring simple poles only, whose intersection numbers can be computed by a generalized version of Residue Theorem \cite{Matsumoto1998IntersectionNF,Mizera:2017rqa}.


Unfortunately this is in general not long true in considering higher genera contributions, for which superspace does not trivially split into fermionic and bosonic degrees of freedom.

Thanks to conformal symmetry of string theory, the integration over a given worldsheet representing an $n$ string scattering process is equivalent to the integration over a Riemann surface of the same genus with $n$ points removed, called punctures. This implies that not all contributions to the amplitude are inequivalent: equivalence classes of $n-$ punctured Riemann surfaces of a given genus $g$ are described by the so called the Moduli space $\M_{g,n}$.
In the bidimensional extension, Feynman diagrams loops become holes in the worldsheet, then the expansion of the string amplitudes in the coupling constant turn to be an expansion over the genera of the worldsheet: higher genera worldsheet integration correspond to higher order contributions. Tree level contributions are then associate to genus $0$ Riemann surfaces, first order contributions to genus $1$ and so on.
   

These different ways are related to the shape of the worlsheet identified by strings in the scattering process; then string amplitudes are expressed as an integration over the metrics of all worldsheets, compatible with the scattering configuration.

In the perturbative approach, string amplitudes are series expanded in the coupling constant; each term of the expansion corresponds to the integration over a Riemann surface of different genus and over all possible positions of the . Due to conformal symmetry, such contributions turn not to be all inequivalent: equivalence classes of $n-$ punctured Riemann surfaces of a given genus $g$ form a space: the Moduli space $\M_{g,n}$.

Differently from QFT, thanks to conformal symmetry, only one diagram contributes to each order of the expansion. 










Using the same notation of \cite{Frellesvig:2019uqt}, let $\{\langle \f_L^{(\mathbb{i})}|\}$ be an element of $H^{\mathbf{i}}_\omega$, and $\{\langle e_i^{i}|\}$ a basis of it, let then denote by $\{\langle \f_L^{(i)}|\}$ a 1-form depending on the $z_i$ variable. 


\begin{equation}
\begin{split}
    \langle \f_L^{(\textbf{n})}|C_R^{(\textbf{n})}] =& \int_{C_R^{(\textbf{n})}}\f_L^{(\textbf{n})}(z_1,..z_n)u = \sum_{i=1}^{\nu_{n-1}}\int_{C_R^{(n)}}\f_{L,i}^{(n)}(z_n)\int_{C_R^{(\textbf{n-1})}}\f_L^{(\textbf{n})}(z_1,..z_n)=\\&=\sum_{i=1}^{\nu_{n-1}}\int_{C_R^{(n)}}\f_{L,i}^{(n)}(z_n)\langle e_i^{(\mathbf{n-1})}|C_R^{(\mathbf{n-1})}], \end{split}
\end{equation}
\nn
where $\nu_{\mathbf{n-1}}= \dim H^{n-1}_\omega$.
\begin{equation}
    d_{z_n} \langle e_i^{(\mathbf{n-1})}|C_R^{(\mathbf{n-1})}]=\mathbf{\Omega}_{ij}^{(n)}\langle e_i^{(\mathbf{n-1})}|C_R^{(\mathbf{n-1})}],
\end{equation}

\begin{equation}
    \nabla_\mathbf{\Omega}^{n}\equiv d_{z_{n}}+\mathbf{\Omega}^{n}
\end{equation}


\begin{equation}
 H^n_\omega \ni \langle \f^{(n)}_L | =\langle e^{(n-1)}| \wedge \langle \langle \f_L \rangle 
\end{equation} 
